Multimodal Federated Learning via Contrastive Representation Ensemble

With the increasing amount of multimedia data on modern mobile systems and IoT infrastructures, harnessing these rich multimodal data without breaching user privacy becomes a critical issue. Federated learning (FL) serves as a privacy-conscious alternative to centralized machine learning. However, existing FL methods extended to multimodal data all rely on model aggregation on single modality level, which restrains the server and clients to have identical model architecture for each modality. This limits the global model in terms of both model complexity and data capacity, not to mention task diversity. In this work, we propose Contrastive Representation Ensemble and Aggregation for Multimodal FL (CreamFL), a multimodal federated learning framework that enables training larger server models from clients with heterogeneous model architectures and data modalities, while only communicating knowledge on public dataset. To achieve better multimodal representation fusion, we design a global-local cross-modal ensemble strategy to aggregate client representations. To mitigate local model drift caused by two unprecedented heterogeneous factors stemming from multimodal discrepancy (modality gap and task gap), we further propose two inter-modal and intra-modal contrasts to regularize local training, which complements information of the absent modality for uni-modal clients and regularizes local clients to head towards global consensus. Thorough evaluations and ablation studies on image-text retrieval and visual question answering tasks showcase the superiority of CreamFL over state-of-the-art FL methods and its practical value.

==> sections/Sentencesmayuse.tex <==
For example, \cite{zhao2022multimodal} targets at real-world IoT scenarios where both uni- and multimodal clients exist, and performs model aggregation for each modality separately while assigning higher weights to models from multimodal clients.

as demanded by complex real-world situation~\citep{zhao2022multimodal} and privacy concerns (illustrated in Figure~\ref{fig:intro}).

Compared with \citet{zhao2022multimodal} that also leverages both uni- and multi-modal data, beyond updating the whole framework to allow larger server model to increase scalability, we also design a more effective and efficient tuning-free aggregation method for multi-modal data.

whereas existing ensemble knowledge transfer algorithms~\citep{zhu2018knowledge,tran2020hydra,nam2021diversity} that transfer and ensemble knowledge from a bag of teachers by \textit{logit} are no longer applicable.

==> sections/intro-origin.tex <==
\section{Introduction}

\jj{Todo: Shorten the first two paragraphs}

% FL and multi-modal FL
% Traditional machine learning systems store massive personal data on a central server to train deep neural nets, which causes severe privacy issues.
Federated Learning (FL)~\citep{mcmahan2017communication}, a decentralized training paradigm that allows parties to collaboratively train models without compromising privacy, has emerged as an alternative to centralized machine learning. 
Most of existing FL methods only consider scenarios where the data transmitting from multiple parties are in the same modality (\textit{e.g.}, image or text).
While with the evolution of modern multi-modal systems (\textit{e.g.}, social networks and other platforms where users can upload and share tagged images, narrated videos and soundtracked memes), there are massive private client data (multi-modal and uni-modal) available on edge devices that can be harnessed to potentially boost the performance of shared \textit{multi-modal systems}, which has raised a surge of growing research interests~\citep{tan2019lxmert,lu2019vilbert,chen2020uniter,li2022grounded} \jj{Add references that actually leverage multimodal customer data}. \qy{I wanted to say MM has raised a surge of interests, to express the necessity to introduce MM into FL}
% Recent state-of-the-art work in multi-modal learning~\citep{singh2022flava} emphasize the importance of taking advantage of unpaired uni-modal data along with multi-modal paired data to enrich representations, which is also in line with the application scenario of FL, \textit{i.e.}, edge devices often hold private data across multiple modalities.
% In practice, however, there are often data across different modalities , \textit{e.g.} images from camera, voice from microphones, text from keyboard input, image-text pairs (maybe weakly correlated) from various APPs like Facebook.

Recently, to leverage client data across various modalities while preserving privacy, different FL approaches~\citep{xiong2022unified,zhao2022multimodal,liu2020federated} have been investigated. \cite{xiong2022unified} first applies a natural extension of FedAvg~\citep{mcmahan2017communication} to multi-modal data. \cite{zhao2022multimodal} targets at real-world FL scenarios with both uni- and multi-modal clients and proposes to assign higher weights to multi-modal clients in aggregation, which is in line with state-of-the-art approach in multi-modal learning~\citep{singh2022flava} that takes advantage of uni-modal data along with multi-modal paired data to enrich representations. 
These methods all adopt FedAvg framework, where server and clients share the same model architecture and communicate with each other by transferring model parameters. This homogeneous design hinders the application of multi-modal FL, due to limited resources on edge devices, which limits the scalability of such systems. 
To make multi-modal FL procedure more practical and applicable, we study this under-explored problem by asking: 

% \begin{center}
    \Romannum{1}. \textit{Can we collaboratively train a larger model over \textbf{heterogeneous} clients (uni- and multi-modal)?} % with different model architectures across various modalities (uni- and multi-modal
% \end{center}

To address this scalability deficiency of model-identical FL framework, \textit{we design an architecture that simultaneously leverages uni- and multi-modal data with a larger server model, to allow heterogeneous multi-modal FL}. Specifically, the server model learns from clients by ensemble knowledge transfer using public data. 
We adopt the setting of \citet{zhao2022multimodal} to leverage both uni- and multi-modal data for real-world application considerations, while we not only update the whole framework to increase scalability, but also design a more effective and efficient aggregation method for multi-modal data that does not need manual tuning.
A few algorithms~\citep{cho2022heterogeneous,cheng2021fedgems} have been proposed for similar heterogeneous purposes. For example, FedET~\citep{cho2022heterogeneous} proposes a Knowledge Distillation (KD)-based FL framework with a large model at server-side and relatively small and applicable models on edge devices.  However, they are all focused on uni-modal FL and difficult to extend to multi-modal setting.  \jj{Explain the difference between our work and \citet{zhao2022multimodal}. } \qy{done, please check}

The main drawback of existing KD-based FL algorithms lies in that they only utilize logits to transfer the knowledge, while for most multi-modal tasks (\textit{e.g.}, image-text retrieval, image/video captioning), logits are no longer applicable. Specifically, image-text retrieval requires \textit{representation} comparison and video captioning generates texts based upon image \textit{representations}. This challenge raises another question:

% \begin{center}
    \Romannum{2}. \textit{Can we train a global multi-modal network that is more applicable and able to handle \textbf{multi-tasks}?} %, \textit{e.g.}, multi-modal retrieval~\citep{long2016composite} and visual question answering~\citep{antol2015vqa}?}
% \end{center}

% Challenges of KD-based FL
% Multimodal \textit{representation} learning and fusion are the bedrocks of multi-modal learning, and methods that leverage large data to learn generalizable representations applicable to multiple downstream tasks now dominate~\citep{zhang2020multimodal}. 
% Given that logits are only applicable to classification tasks, these methods have limited generality and are no longer viable to many multi-modal tasks that essentially require representations alignment, like retrieval, image-text matching, as well as image captioning that operate on image representations. 
To address this, \textit{we propose to transmit low-dimensional representations instead of logits between server and clients in multi-modal FL setting}. Representations are usually high-dimensional and contextual, and contain more granular information than logits. Besides, multi-modal representation is effective in generalization to various downstream tasks~\citep{devlin2018bert,chen2020uniter}, which also adheres to the spirit of recent progress in foundation models~\citep{bommasani2021opportunities}.

% To use representations instead of logits, diverse representations generated by different clients need to be aggregated for ensemble transfer. 
% For logits, there exists many aggregation strategies~\citep{cho2022heterogeneous,cheng2021fedgems} based on the distributional nature of logits.
% For example, FedET~\citep{cho2022heterogeneous} believes that logits with higher variance should be up-weighted because models are more confident about these predictions. 
% % , FedGEMS~\citep{cheng2021fedgems} entropy. 
% But such logit-specific aggregation strategies are not suitable for representation, as their contextual meanings are different. \jj{Different in what way?} 
%As a naive approach, we can average all representations for knowledge transfer, while we still want to absorb the knowledge learned across heterogeneous clients from massive private user data more efficiently. 


%In addition to typical non-i.i.d. problem, `modality gap' and `task gap' issues cause
Another big challenge in multi-modal FL is harsher model drift~\citep{karimireddy2020scaffold} between clients. For example, 
Uni-modal clients trained under single modality (\textit{e.g.} image) have never seen data from other modalities (\textit{e.g.}, text) in the training procedure, while multi-modal clients are trained with multi-modality data (\textit{e.g.}, image-text pairs). We call this `\textit{modality gap}' between clients. 
Moreover, different clients might be trained for different tasks, \textit{e.g.}, image classification for uni-modal image clients and image-text retrieval for multi-modal clients. We call this `\textit{task gap}' between clients. 
Both gaps cause unprecedented model drift problems in multi-modal FL. %\textit{How to \textbf{mitigate local model drift} in multi-modal scenario} is a second challenge in heterogeneous multi-modal federated learning.
That raises a new challenge:

% \begin{center}
    \Romannum{3}. \textit{How to mitigate local model drift in multi-modal FL?}
% \end{center}

To alleviate `modality gap', \textit{we propose an inter-modal contrastive objective} that performs cross-modality contrasts using public data in the local training phase, to complement information of the absent modality for uni-modal clients. To tackle `task gap', \textit{we propose an intra-modal contrastive objective} that contrasts local representations to their corresponding global ones in each separate modality, to regularize models heading towards the global 
consensus~\citep{li2019fedmd}.\jj{What's global commonsense?} \qy{sry, it should be global `consensus', which can be seen as a global agreement that has the least bias and drift.}

\jj{Todo: Shorten the following paragraphs into a summary of contributions} \qy{not done.}

To address the above challenges, we propose \name, a cross-modal contrastive Multi-Modal Federated Learning framework with Feature (Representation)-Level knowledge transfer. 
Multimodal learning aims to learn joint representations that semantically correlated images and texts share. 
% ToDo, written by Yimu
% MM\underline{FL}$^2$ is a heterogeneous architecture that enables different model employed on the server and client sides, and aims to learn joint representations that semantically correlated images and texts share. 
% Besides, inspired by contrastive learning, we design a novel cross-modal contrastive score that measures the importance of representations generated by different clients and use this score as the weights of KD to ensemble the representations and knowledge. 
Under the guidance of this goal, we first design a criterion to evaluate quality of representations for effective ensemble transfer. We hope local representations that $1)$ better match the paired representations generated by the global model, and $2)$ less approximate the unpaired public representations, to play a more critical role in ensemble, and design a cross-modal contrastive score as weight for ensemble transfer from the inspiration of contrastive learning. 
The proposed weighting score brings us two benefits: $1)$ we can identify representations that align better with their paired data and assign them higher weights to facilitate cross-modal interactions; $2)$ as contrasting to global representations that serve as consensus, we can filter out outliers that suffers too much from the domain gap and model drift. 
To further reduce local model drift, we introduce inter- and intra-modal contrastive objective to regularize local training. 

Our contributions are summarized below: (TODO, not written)
\begin{itemize}
    \item \name is the first heterogeneous multi-modal FL method which enables different server and client settings and the first multi-modal FL method to utilize representations to transfer knowledge between clients and the server.
    \item The proposed contrast-based score for aggregation and intra-\&inter-modal contrasting for minimizing model drift and 'task gap' introduced by uni- and multi-modal clients.
    \item \name outperforms others multi-modal and extensions of uni-modal FL algorithms on image-text retrieval and visual question answering tasks.
\end{itemize}

% [Think globally] requires all clients to have data from all modalities and aligned, which is not practical in real-world application. A more practical setting is uni-modal, multi-modal

% our method does not share representations of local data to the server.

% [IoT] also work on clients with different local data modalities, while it investigate less on how to aggregate information from clients across different modalities, which are more heterogeneous than traditional FL settings.
% The local training of [IoT], which may have a more severe local model drift, which may impedes the performance.


==> sections/intro-v2-3questions.tex <==
\section{Introduction}

% FL and multi-modal FL
% Traditional machine learning systems store massive personal data on a central server to train deep neural nets, which causes severe privacy issues.
Federated Learning (FL)~\citep{mcmahan2017communication}, a decentralized training paradigm that allows parties to collaboratively train models without compromising privacy, has emerged as an alternative to centralized machine learning. 
Most of existing FL methods only consider scenarios where the data transmitting from multiple parties are of the same modality (\textit{e.g.}, image or text).
With the evolution of modern multi-modal systems such as social networks where users can upload and share tagged images and narrated videos, there is a massive amount of private data in multi-modal forms available on edge devices that can be harnessed~\citep{tan2019lxmert,lu2019vilbert,chen2020uniter,li2022grounded}. 
% Recent state-of-the-art work in multi-modal learning~\citep{singh2022flava} emphasize the importance of taking advantage of unpaired uni-modal data along with multi-modal paired data to enrich representations, which is also in line with the application scenario of FL, \textit{i.e.}, edge devices often hold private data across multiple modalities.
% In practice, however, there are often data across different modalities , \textit{e.g.} images from camera, voice from microphones, text from keyboard input, image-text pairs (maybe weakly correlated) from various APPs like Facebook.

To effectively leverage private client data across various modalities while preserving privacy, a new multi-modal FL landscape poses three major challenges in terms of model architecture, targeted tasks and data diversity:   
(\Romannum{1}) Can we collaboratively train a larger server model over \textit{heterogeneous} clients? Here, `heterogeneous' refers to not only diverse model architectures but also different multi-modality data formats across clients, as shown in Figure~\ref{fig:intro}.
(\Romannum{2}) Can we train a single global network that is capable of handling \textit{diverse multi-modal tasks (e.g., image-text retrieval, visual question answering)}? 
(\Romannum{3}) How to mitigate \textit{local model drift} caused by modality gap?


Recently, a few algorithms~\citep{cho2022heterogeneous,cheng2021fedgems} have been developed for handling heterogeneous clients with different architectures. For example, FedET~\citep{cho2022heterogeneous} proposes a Knowledge Distillation (KD) based framework with a large model at server-side and relatively small and deployable models on edge devices. However, they are all focused on uni-modal FL and difficult to extend to multi-modal setting. On the other hand, there have been some early attempts at applying FL to multi-modal tasks~\citep{xiong2022unified,zhao2022multimodal,liu2020federated}. For example, \cite{zhao2022multimodal} targets at real-world FL scenarios with both uni- and multi-modal clients, and proposes to assign higher weights to multi-modal clients in aggregation.
%, which is in line with state-of-the-art approach in multi-modal learning~\citep{singh2022flava} that takes advantage of uni-modal data along with multi-modal paired data to enrich representations. 
However, these methods all adopt FedAvg framework, where the server and clients share the same model architecture % and communicate with each other by transferring model parameters. 
with a homogeneous design, limiting the scale of the server model. 
To address this scalability \yang{try avoid "scalable/scalability" since it also means large number, i.e., millions of clients whereas our experiments are not very large.} and homogeneity deficiency of FL algorithms, we design a novel contrastive multi-modal federated learning framework \name, which \textit{simultaneously leverages uni- and multi-modal data across heterogeneous clients} to allow a larger server model. Specifically, the server model learns from clients via ensemble knowledge transfer on public data with a tuning-free aggregation mechanism that works for diverse client networks. (Figure~\ref{fig:intro})
%Compared with \citet{zhao2022multimodal} that also leverages both uni- and multi-modal data, beyond updating the whole framework to allow larger server model to increase scalability, we also design a more effective and efficient tuning-free aggregation method for multi-modal data.

%To make multi-modal FL procedure more practical and applicable, we study this under-explored problem by asking: 
% % \begin{center}
%     \Romannum{1}. \textit{Can we collaboratively train a larger model over \textbf{heterogeneous} clients (uni- and multi-modal)?} % with different model architectures across various modalities (uni- and multi-modal
% % \end{center}

% To address this scalability deficiency of model-identical FL framework, \textit{we design an architecture that simultaneously leverages uni- and multi-modal data with a larger server model, to allow heterogeneous multi-modal FL}. Specifically, the server model learns from clients by ensemble knowledge transfer using public data. 
% We adopt the setting of \citet{zhao2022multimodal} to leverage both uni- and multi-modal data for real-world application considerations, while we not only update the whole framework to increase scalability, but also design a more effective and efficient aggregation method for multi-modal data that does not need manual tuning.

Existing KD-based FL algorithms all utilize logits to transfer knowledge, while for most multi-modal tasks (\textit{e.g.}, image-text retrieval, image/video captioning), logits are no longer applicable, as these cross-modality tasks typically operate on fused vision-and-language representation level.  
%For example, image-text retrieval requires \textit{representation} comparison, and video captioning generates texts based upon image \textit{representations}. 
%This challenge raises another question:
% % \begin{center}
%     \Romannum{2}. \textit{Can we train a global multi-modal network that is more applicable and able to handle \textbf{multi-tasks}?} %, \textit{e.g.}, multi-modal retrieval~\citep{long2016composite} and visual question answering~\citep{antol2015vqa}?}
% % \end{center}
% Challenges of KD-based FL
% Multimodal \textit{representation} learning and fusion are the bedrocks of multi-modal learning, and methods that leverage large data to learn generalizable representations applicable to multiple downstream tasks now dominate~\citep{zhang2020multimodal}. 
% Given that logits are only applicable to classification tasks, these methods have limited generality and are no longer viable to many multi-modal tasks that essentially require representations alignment, like retrieval, image-text matching, as well as image captioning that operate on image representations. 
To address this, we propose to \textit{transmit low-dimensional representations instead of logits} between server and clients. Representations are usually high-dimensional and contextual, and contain more granular information than logits. Besides, multi-modal representation is critical in generalization to various downstream tasks~\citep{devlin2018bert,chen2020uniter}, which adheres to the spirit of recent trend in foundation models~\citep{bommasani2021opportunities}. \yang{I don't think we need to stress this point as our novelty in introduction since it is a natural choice . Just mention it in methods.}

To effectively aggregate representations, we propose a global-local cross-modal contrastive score for weighting, to filter out outliers that drift too much by contrasting \textit{local} representations to \textit{global} ones, and pick out outstanding candidates that match better to their paired partners by contrasting to representations from \textit{another modality}.
% To use representations instead of logits, diverse representations generated by different clients need to be aggregated for ensemble transfer. 
% For logits, there exists many aggregation strategies~\citep{cho2022heterogeneous,cheng2021fedgems} based on the distributional nature of logits.
% For example, FedET~\citep{cho2022heterogeneous} believes that logits with higher variance should be up-weighted because models are more confident about these predictions. 
% % , FedGEMS~\citep{cheng2021fedgems} entropy. 
% But such logit-specific aggregation strategies are not suitable for representation, as their contextual meanings are different. \jj{Different in what way?} 
%As a naive approach, we can average all representations for knowledge transfer, while we still want to absorb the knowledge learned across heterogeneous clients from massive private user data more efficiently. 


%In addition to typical non-i.i.d. problem, `modality gap' and `task gap' issues cause
Another big challenge in multi-modal FL is harsher model drift~\citep{karimireddy2020scaffold} between clients. For example, 
uni-modal clients trained under single modality (\textit{e.g.} image) have never seen data from other modalities (\textit{e.g.}, text) in the training procedure, while multi-modal clients are trained with multi-modality data (\textit{e.g.}, image-text pairs). We call this `\textit{modality gap}' between clients. 
Moreover, different clients might be trained for different tasks, \textit{e.g.}, image classification task for uni-modal clients and image-text retrieval task for multi-modal clients. We call this `\textit{task gap}' between clients. 
Both gaps cause unprecedented model drift problems in FL training. %\textit{How to \textbf{mitigate local model drift} in multi-modal scenario} is a second challenge in heterogeneous multi-modal federated learning.

% That raises a new challenge:
% % \begin{center}
%     \Romannum{3}. \textit{How to mitigate local model drift in multi-modal FL?}
% % \end{center}

To reduce this model drift, we introduce two novel contrastive objectives to regularize local training. An \textit{inter-modal contrastive objective} is designed to mitigate `modality gap', by performing cross-modality contrasts using public data in the local training phase, which complements for the information of the absent modality in uni-modal clients. To tackle `task gap', an \textit{intra-modal contrastive objective} is proposed to contrast local representations to their corresponding global ones in each modality, to regularize models heading towards the global consensus~\citep{li2019fedmd}.

%To address the above challenges, we propose \name, a cross-modal contrastive Multi-Modal Federated Learning framework with Feature (Representation)-Level knowledge transfer. 
%Multimodal learning aims to learn joint representations that semantically correlated images and texts share. 
% ToDo, written by Yimu
% MM\underline{FL}$^2$ is a heterogeneous architecture that enables different model employed on the server and client sides, and aims to learn joint representations that semantically correlated images and texts share. 
% Besides, inspired by contrastive learning, we design a novel cross-modal contrastive score that measures the importance of representations generated by different clients and use this score as the weights of KD to ensemble the representations and knowledge. 

%Under the guidance of this goal, we first design a criterion to evaluate quality of representations for effective ensemble transfer. We hope local representations that $1)$ better match the paired representations generated by the global model, and $2)$ less approximate the unpaired public representations, to play a more critical role in ensemble, and design a cross-modal contrastive score as weight for ensemble transfer from the inspiration of contrastive learning. 
%The proposed weighting score brings us two benefits: $1)$ we can identify representations that align better with their paired data and assign them higher weights to facilitate cross-modal interactions; $2)$ as contrasting to global representations that serve as consensus, we can filter out outliers that suffers too much from the domain gap and model drift. 
%\jj{Move these detailed explanations of the contrastive methods to the Method section}
%To further reduce local model drift, we introduce inter- and intra-modal contrastive objective to regularize local training. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.45]{images/intro.pdf}
    \caption{Overview}
    \label{fig:intro}
\end{figure}

In summary, the contributions of this work are three-fold:
\begin{itemize}
    \item \name\ is the first heterogeneous multi-modal FL framework to support different server and client architectures. Experiments show that \name\ outperforms other FL systems in multi-modal setting in terms of both model performance and communication cost.
    \item \name\ is the first FL method to utilize granular representations instead of logits to transfer knowledge between clients and the server, and we design a novel global-local cross-modal aggregation strategy for representation. Experiments show that our aggregation strategy achieves superior performance to other ensemble strategies commonly used in FL.
    \item The proposed inter-modal and intra-modal contrasting objectives effectively minimize local model drift introduced by cross-modality data discrepancy.
    %\item \name outperforms others multi-modal and extensions of uni-modal FL algorithms on image-text retrieval and visual question answering tasks.
\end{itemize}

% [Think globally] requires all clients to have data from all modalities and aligned, which is not practical in real-world application. A more practical setting is uni-modal, multi-modal

% our method does not share representations of local data to the server.

% [IoT] also work on clients with different local data modalities, while it investigate less on how to aggregate information from clients across different modalities, which are more heterogeneous than traditional FL settings.
% The local training of [IoT], which may have a more severe local model drift, which may impedes the performance.

\yang{I find the introduction is a little scattered and hard to follow. So I suggest re-org a little with the following logic: 1. most FL works are uni-modal. 2. Multi-modal (MM) tasks are very common , however data are generated from heterogeneous edge devices and big model is built on centralized server. (Mobile example, may add another smart home example) 3. With increasing privacy concerns, it is desirable to enable federated learning of large MM models with heterogeneous data and device at edge. 4. The past FL works either consider federated learning of large models with uni-modal data, or per-modality model aggregation of modality-dependent models at edge, which does not allow for heterogeneous model architecture within each modality and are subject to model inversion attacks. 5. Therefore we design a novel MM FL framework to address these challenges. 6.The contributions/features of our framework: We enable a KD-based MM FL framework which allows for heterogeneous modality and model architecture at the edge whiling only communicating private knowledge on public dataset without revealing private models;  We develop cross-modal contrastive and aggregation strategy to address model drift and achieve better representation learning and aggregation performance; Our framework enables larger model training at the server which is required for challenging MM tasks and pave ways for federated learning of even more challenging tasks, such as foundation models at the edge.}

\yang{please also consider to re-org abstract based on this.}
